Infrared: A Meta Bug Detector

The recent breakthroughs in deep learning methods have sparked a wave of interest in learning-based bug detectors. Compared to the traditional static analysis tools, these bug detectors are directly learned from data, thus, easier to create. On the other hand, they are difficult to train, requiring a large amount of data which is not readily available. In this paper, we propose a new approach, called meta bug detection, which offers three crucial advantages over existing learning-based bug detectors: bug-type generic (i.e., capable of catching the types of bugs that are totally unobserved during training), self-explainable (i.e., capable of explaining its own prediction without any external interpretability methods) and sample efficient (i.e., requiring substantially less training data than standard bug detectors). Our extensive evaluation shows our meta bug detector (MBD) is effective in catching a variety of bugs including null pointer dereference, array index out-of-bound, file handle leak, and even data races in concurrent programs; in the process MBD also significantly outperforms several noteworthy baselines including Facebook Infer, a prominent static analysis tool, and FICS, the latest anomaly detection method.

==> evadatarace.tex <==
% !TEX root = ./main.tex  

The six types of bugs selected from defect4j are related to the bug types in our training set. In order to evaluate the effectiveness of the tool in the unseen bug types, we use the second dataset JBench, which contains a variety of data race bugs. There are three main reasons why we choose to evaluate on the data race. First, the data race is a type of bug that the model has not learned at all, and it can effectively show the generalization ability of the model. Second, data race detection is very important, and data race existence has caused great losses to software. Third, data race is difficult to detect, whether it is for static analysis or dynamic testing.

There are six open source projects in JBench and total 781 data race bugs. But we cannot use all these bugs for evaluation, because some bugs are triggered in library methods and we can not generation the PDG graph of library methods. Some bugs are in the same methods but we treat one method as one bug. So there are total of 275 bugs can be used for our evaluation after filtering. We compare \tool against Facebook Infer and FICS on data race dataset.

In order to detect data race, it is critical to find shared variable. In this paper, we follow the algorithm of shared variable discovery proposed by~\citet{kahlon2007fast}. 
The algorithm is to detect complete update sequences from $p$ to $q$ (\eg $ p_1 = p; p_2 = p_1; \dots ; q = p_k$)  that are followed by the modification of a variable accessed via $q$ (\eg $q$-$>m = val;$), where $p$ either points to a global
variable or is passed as a parameter to an API function. 
Any variable is declared as shared if (1) it is propagated from a complete update sequences; and (2) assigned by a local variable or an expression other than simple propagation of a data value. 

\begin{figure}[h!]
	\centering
	\captionsetup{skip=4pt}

	\parbox{.70\linewidth}{
  	\lstset{style=mystyle}
		\lstinputlisting[morekeywords={Object, String}, numbers=left, stepnumber=1, xleftmargin=2em, frame=single, framexleftmargin=1.5em]{Code/examplerace2.java}
	}
	\caption{An example of data race program.}
	\label{fig:racesource} 
\end{figure}

\begin{figure}[h!]
	\centering
	\captionsetup{skip=4pt}

	\includegraphics[height=6cm]{pic/datarace.pdf}
	\caption{The representation of data race program. We add a data dependency edge between the same global variables to indicate that there is a data flow between them.}
	\label{fig:racerep}
\end{figure}

Figure ~\ref{fig:racesource} depicts an example of real data race bug comes from ~\citet{10.1145/966049.781528}. In this example, the main thread starts a child thread and trys to terminate it. When line 11 (\ie \textit{main.childThread = null}) runs between line 8 (\ie \textit{if(childThread != null)}) and line 9 (\ie \textit{childThread.interrupt()}), it will cause a null pointer dereference, because only one lock cannot guarantee the mutual operations of \textit{childThread}. So there is a potential data race and this is obviously a missing statements bug.



In a Java program, if a class \textit{extends} the \textit{Thread} class, when the \textit{start()} method of this class is called, the \textit{run()} method of this class will concurrently execute. We can find that Main.execute() is the caller of ChildThread().run() and they belong to different threads base on this knowlodge. Through pointer analysis, we can also find that \textit{main.childThread} in \textit{ChildThread.run()} and \textit{childThread} in \textit{Main.execute()} are the same shared variable. 

% Given the data race program, we first found a shared variable \texttt{s} in method \texttt{foo} according to a complete update sequence $ s = new Obj(); a = s; f = a; x = f; x1  = x; x1.do_something()$. Then, we represent the program by \wyc{explain how we construct the graph.} 


In order to indicate that there is a possible data race between the two use points of the same global variable, we use an data dependency edge to connect the two use points of the same global variable in the program dependency graph, as Figure ~\ref{fig:racerep} shows. 

Since FICS claims to be able to detect any type of bug, we conducted this experiment with FICS. As long as the FICS report contains any variable related to the data race, we think that FICS has reported this bug. Through experiments, we found that \tool, Facebook Infer, and FICS have reported 40, 2, and ? bugs respectively. The results showing that the effct of \tool in the data race testing set are close to Facebook Infer and far better than FICS. Obviously, \tool can detect more complex bugs that have never been seen in training set. Even though data race is the bug that the model has not learned, there are some commonalities in data race. If there is data race due to no lock operation, we can regard it as a missing statements bug. If the data race is caused by the wrong lock position, we can treat it as a statement position error. If the wrong lock is used, we can treat it as a variable misuse.

% \begin{table}[htbp]
% 	\caption{Compare \tool against Infer and FICS on data race.}
% 	\begin{tabular}{c|c|c}
% 		\hline
%     & TP& FN \\\hline
% 		Facebook Infer& & \\\hline
% 		FICS& & \\\hline
% 		\tool (Top-5)& & \\\hline
% 		\tool (Top-10)& & \\\hline
% 		\tool (Top-15)& & \\\hline
% 	\end{tabular}
% 	\label{tab:dataraceres}
% \end{table}

